A nonparametric doubly robust test for a continuous treatment effect

The vast majority of literature on evaluating the significance of a treatment effect based on observational data has been confined to discrete treatments. These methods are not applicable to drawing inference for a continuous treatment, which arises in many important applications. To adjust for confounders when evaluating a continuous treatment, existing inference methods often rely on discretizing the treatment or using (possibly misspecified) parametric models for the effect curve. Recently, Kennedy et al. (2017) proposed nonparametric doubly robust estimation for a continuous treatment effect in observational studies. However, inference for the continuous treatment effect is a harder problem. To the best of our knowledge, a completely nonparametric doubly robust approach for inference in this setting is not yet available. We develop such a nonparametric doubly robust procedure in this paper for making inference on the continuous treatment effect curve. Using empirical process techniques for local U- and V-processes, we establish the test statistic's asymptotic distribution. Furthermore, we propose a wild bootstrap procedure for implementing the test in practice. We illustrate the new method via simulations and a study of a constructed dataset relating the effect of nurse staffing hours on hospital performance. We implement our doubly robust dose response test in the R package DRDRtest on CRAN.

==> input/conc.tex <==

\begin{mylongform}
  \begin{longform}

    We have developed a new doubly robust procedure for testing whether a treatment
    causally affects a response when the treatment is continuous.
    This case, where treatment is continuous, involves more mathematical hurdles than  the cases of binary or discrete treatments,
    and the former case is generally still much less developed than the
    latter cases.


  \end{longform}
\end{mylongform}

Some brief directions for interesting and valuable future research are as follows.
% \remCRD{I am not sure if I understand this aspect very well yet, but I
% do suspect we should include some comments.}
Our test statistic is based on a certain pseudo-outcome, $\xi$.
This pseudo-outcome leads to estimators that are analogous to certain
doubly robust estimators in the discrete or binary case
(e.g., \citep{robins2001comment}); but it is well-known in the discrete case that
such estimators can perform poorly when inverse probability weights are
highly variable, see for instance \cite{robins2001comment}.
In the case of
continuous treatments, the existence of one or more intervals of treatment
values that have low (true) propensity function values (i.e., a set of
covariates/confounders for which some interval of treatment values is
unlikely) is quite common.
In the supplement, we plot the (estimated) propensity scores, which we truncated to be $0.01$ if they fell below that value,  from our analysis of the nursing hours dataset, in Figure~\ref{supp:fig:ps-plot}.
The plot makes it clear that indeed the propensity scores are commonly quite small, so we are in the setting of highly variable inverse weights.
\begin{mylongform}
  \begin{longform}
    (Note that although $\xi$ is defined by using weights
    $\int_{\mc L} \pi(a | \bs l) dP(\bs l) / \pi(a | \bs L)$ rather than
    $ 1 / \pi(a | \bs L)$ (the latter being slightly more formulaically
    directly connected to the discrete case), this does not fundamentally
    change the issue.)
  \end{longform}
\end{mylongform}
Thus an important direction for future research, which may be even more important for the case of continuous treatments than it is in the case of discrete treatments, is what to do when the (true or estimated) propensity function takes on very low values.  One direction is to consider modifying $\xi$ by re-weighting the inverse probability weights so the weights sum to 1 (see display (1) in
\cite{robins2001comment}).
\remCRD{ Does ``sum to 1'' make sense?  (They are already normalized by an integral.).}
%% , although such $\xi$ may still be highly variable.
Another direction is to attempt to pursue methods analogous to those
yielding the ``boundedness'' property described in Section~4.1 of
\cite{robins2001comment}.



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../drtest-main"
%%% End:

